On the complexity of linear systems: an approach via rate distortion theory and emulating systems

We define the complexity of a continuous-time linear system to be the minimum number of bits required to describe its forward increments to a desired level of fidelity, and compute this quantity using the rate distortion function of a Gaussian source of uncertainty in those increments. The complexity of a linear system has relevance in control-communications contexts requiring local and dynamic decision-making based on sampled data representations. We relate this notion of complexity to the design of attention-varying controllers, and demonstrate a novel methodology for constructing source codes via the endpoint maps of so-called emulating systems, with potential for non-parametric, data-based simulation and analysis of unknown dynamical systems.

==> cmds.tex <==

%%%%%%%%%%%%%%%%%%%%%%%
%: Custom math commands 

% Vector superscript commands
\makeatletter
\def\my@overarrow@#1#2#3{\vbox{\ialign{##\crcr #1#2\crcr \noalign{\kern-\p@\nointerlineskip}$\m@th \hfil #2#3\hfil $\crcr}}}

%\newcommand{\amsvect}{%
	%  \mathpalette {\my@overarrow@\vectfill@}}
%\def\vectfill@{\arrowfill@\relbar\relbar{\raisebox{-3.81pt}[\p@][\p@]{$\mathord\mathchar"017E$}}}
%
%\newcommand{\amsvectb}{%
	%  \mathpalette {\my@overarrow@\vectfillb@}}
%\newcommand{\vecbar}{%
	%  \scalebox{0.8}{$\relbar$}}
%\def\vectfillb@{\arrowfill@\vecbar\vecbar{\raisebox{-4.35pt}[\p@][\p@]{$\mathord\mathchar"017E$}}}
%\makeatother

% New paragraph section macros
\newcommand{\skippar}{\vskip\topsep\noindent}
\newcommand{\parsec}[1]{%
	\vskip\topsep\noindent\textit{#1}.\hspace{.5\parindent}}
\newcommand{\parsecnoskip}[1]{%
	\noindent\textit{#1}.\hspace{.5\parindent}}

% Mathbb
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}

% Caligraphic font
\newcommand{\J}[1]{\ensuremath{\mathcal{J}^{(#1)}}}

% Serif font
\newcommand{\Cinf}{\ensuremath{\mathsf{C}^\infty}}
\newcommand{\Vect}{\ensuremath{\mathsf{Vec}}}
\newcommand{\Lin}{\ensuremath{\mathsf{Lin}}}
\newcommand{\Pol}{\ensuremath{\mathsf{Pol}}}
\newcommand{\Ham}{\ensuremath{\mathsf{Ham}}}
\newcommand{\GL}[1]{\ensuremath{\mathsf{GL}_{#1}}}
\newcommand{\SL}[1]{\ensuremath{\mathsf{SL}_{#1}}}
\newcommand{\In}{\ensuremath{\mathsf{In}}}

% Fraktur font
\newcommand{\tauts}{\ensuremath{\mathfrak{s}}}
\newcommand{\s}{\ensuremath{\mathfrak{s}}}
\newcommand{\liesl}[1]{\ensuremath{\mathfrak{sl}_#1}}
\newcommand{\g}[1]{\ensuremath{\mathfrak{g}_{#1}}}

% New symbols and macros
\newcommand{\G}{Gr\"{o}bner}
\newcommand{\mtrx}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\vctr}[1]{\ensuremath{\begin{pmatrix} #1 \end{pmatrix}}}
% \newcommand{\st}{\ensuremath{\  \big|\  }}
\newcommand{\given}{\ensuremath{\,\big|\,}}
\newcommand{\suchthat}{\ensuremath{\  \big|\  }}
\newcommand{\rightexp}{\ensuremath{\overset{\longrightarrow}{\exp}}}
\newcommand{\del}[2]{\ensuremath{\frac{\partial#1}{\partial#2}}}
\newcommand{\deltwo}[2]{\ensuremath{\frac{\partial^2#1}{\partial#2^2}}}
\newcommand{\indel}[2]{\ensuremath{\partial#1/\partial#2}}
\newcommand{\indeltwo}[2]{\ensuremath{\partial^2#1/\partial#2^2}}
\newcommand{\RegAbExt}{\ensuremath{W}}
\newcommand{\CharLineBundle}{\ensuremath{\mathcal{C}}}
\newcommand{\MaxClass}{\ensuremath{\mathcal{R}}}
\newcommand{\SAb}[2]{\ensuremath{(#1^2)^\perp(#2)\backslash(#1^3)^\perp(#2)}}
\newcommand{\I}{\ensuremath{\mathcal{I}}} % vanishing ideal
\newcommand{\V}{\ensuremath{\mathcal{V}}} % set of zeroes
\newcommand{\Att}[2]{\ensuremath{\mathcal{A}_{#1}^{#2}}}

\newcommand{\indpt}{\perp\!\!\!\!\perp} % statistical independence symbol
\newcommand{\msout}[1]{\text{\sout{\ensuremath{#1}}}} % math strikeout, for presentations

\let\mod\oldmod
\newcommand{\mod}{\ensuremath{\ \mathrm{ mod }\ }}
%\DeclareMathOperator{\mod}{mod}

\newcommand{\vv}[1]{\vec{\mkern2mu#1}}
\newcommand{\vu}{\ensuremath{\vv{u}}}
\newcommand{\vh}{\ensuremath{\vv{h}}}
%\newcommand{\vvv}[1]{\vec{#1\mkern2mu}}

% Plain text
\newcommand{\dm}{\ensuremath{\text{d}}}
\newcommand{\wt}{\ensuremath{\text{wt}}}
\newcommand{\extd}{\ensuremath{ \, \text{d}}}
\newcommand{\ord}{\ensuremath{\text{ord}}}

% Math operators
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\mathspan}{span}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Vctr}{Vec}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Ab}{Ab}
\DeclareMathOperator{\RAb}{RAb}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Alt}{Alt}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Cov}{Cov}

% Math theorem environments
\theoremstyle{plain}% default
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{prob}{Problem}

\theoremstyle{remark}
\newtheorem*{rmk}{Remark}
% \newtheorem*{note}{Note}
\newtheorem{case}{Case}


